Laziness Is a Virtue When It Comes to Compositionality in Neural Semantic Parsing

Nearly all general-purpose neural semantic parsers generate logical forms in a strictly top-down autoregressive fashion. Though such systems have achieved impressive results across a variety of datasets and domains, recent works have called into question whether they are ultimately limited in their ability to compositionally generalize. In this work, we approach semantic parsing from, quite literally, the opposite direction; that is, we introduce a neural semantic parsing generation method that constructs logical forms from the bottom up, beginning from the logical form's leaves. The system we introduce is lazy in that it incrementally builds up a set of potential semantic parses, but only expands and processes the most promising candidate parses at each generation step. Such a parsimonious expansion scheme allows the system to maintain an arbitrarily large set of parse hypotheses that are never realized and thus incur minimal computational overhead. We evaluate our approach on compositional generalization; specifically, on the challenging CFQ dataset and three Text-to-SQL datasets where we show that our novel, bottom-up semantic parsing technique outperforms general-purpose semantic parsers while also being competitive with comparable neural parsers that have been designed for each task.

==> content/introduction.tex <==
\section{Introduction}
\label{introduction}
% In this work, we consider the task of semantic parsing, i.e., the task of parsing a natural language utterance into a structured logical form \cite{zelle1996learning}. The earliest learning-based approaches to semantic parsing would induce probabilistic grammars that defined how words and phrases could be combined into formal meaning representations \cite{zettlemoyer2005learning,Kate2005LearningTT,kwiatkowski2011lexical}. While effective in closed domains with limited vocabularies, such approaches were often challenging to train and difficult to scale to settings involving greater breadth, e.g., WebQuestions \cite{berant2013semantic}. With the advent of deep learning and its application to natural language processing \cite{mikolov2013distributed,sutskever2014sequence}, the semantic parsing community shifted towards neural-based methods for their ability to flexibly handle language and the ease with which they could be trained.

Compositionality is inherent to natural language, with the meaning of complex text or speech understood through the composition of constituent words and phrases \cite{montague1973proper}. The ability to process such compositionality is a key feature of human intelligence and is {\color{red}suspected} to play a significant role in why humans are so efficient at generalization \cite{lake2017building}. For instance, having observed the usage of phrases like "edited by" and "directed by" in isolation, a human would be able to easily understand the question "Was Toy Story edited by and directed by John Lasseter?". This ability to take individual components and combine them together in novel ways is known as \textit{compositional generalization}.

Compositional generalization has been identified as a major point of weakness in neural methods for semantic parsing \cite{lake2018generalization,higgins2018scan}. Accordingly, this deficiency has been taken up as a challenge by the machine learning community, leading to a slew of methods \cite{liu2021learning,herzig2021unlocking,gai2021grounded} and datasets \cite{keysers2019measuring,kim2020cogs} targeted towards compositional generalization. However, while there has been progress in determining factors that allow systems to compositionally generalize \cite{furrer2020compositional,oren2020improving}, there yet remains gaps in our understanding as to why these neural models fail.

% In this work, we consider the task of semantic parsing, i.e., the task of parsing a natural language utterance into a structured logical form \cite{zelle1996learning}. Neural-based methods have become a dominant paradigm within the semantic parsing community, 
% %largely due to the ease with which they can be trained and their ability to flexibly handle the variety inherent to natural language. Recent years have seen an explosion of promising results for neural approaches to semantic parsing, 
% with recent years seeing applications of such methods ranging from Knowledge Base Question Answering~\cite{kapanipathi2021leveraging,naseem2021semantics} to Text-to-SQL~\cite{scholak2021picard,gan2021natural}. These approaches almost universally follow a two-stage encoder-decoder framework \cite{sutskever2014sequence}. In the first stage, natural language input (e.g., a question expressed in text) is encoded by a neural sequence model into a real-valued vector representation, and in the second, the encoded representation is used by a neural decoder to generate a logical expression. Most commonly, the strategy followed by neural decoders is to generate logical forms from the top down in an autoregressive fashion \cite{dong-lapata-2016-language,xiao-etal-2016-sequence,AlvarezMelis2017TreestructuredDW,krishnamurthy-etal-2017-neural,dong-lapata-2018-coarse}. That is, they output a linearization of the target logical form's abstract syntax tree, beginning from the root of the tree, where the generation of each token is conditioned on both the input text as well as the entire sequence of previously generated tokens. 

% While autoregressive, top-down neural semantic parsers currently hold the state-of-the-art on many challenging datasets~\cite{berant2013semantic,pasupat2015compositional,Yu2018SpiderAL}, they have been shown to fail in systematic ways~\cite{johnson2017clevr}. Most notably, such systems have yet to definitively demonstrate an ability to compositionally generalize \cite{lake2018generalization,higgins2018scan}. This deficiency has been taken up as a challenge by the machine learning community, leading to a slew of methods \cite{liu2021learning,herzig2021unlocking,gai2021grounded} and datasets \cite{keysers2019measuring,kim2020cogs} targeted specifically towards the problem of compositional generalization. However, while there has been progress in determining factors going into compositional generalization \cite{furrer2020compositional,oren2020improving}, there yet remains gaps in our understanding as to why these neural models fail.


\begin{figure*}[t]
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=0.85\textwidth]{figures/td_gen.png}
\caption{Top-down decoding (nodes drawn with dotted lines are those being generated)}
\label{fig:td_gen}
\end{subfigure}
\vskip 0.05in
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=0.85\textwidth]{figures/bu_gen.png}
\caption{Bottom-up decoding (nodes drawn with dotted lines are those being generated)}
\label{fig:bu_gen}
\end{subfigure}
\caption{Top-down versus bottom-up decoding strategies for the Geoquery question "What rivers are in s0?"}
\label{fig:td_bu_diff}
\end{figure*}


%In this paper, we posit that the failure of traditional neural semantic parsers to compositionally generalize is in part due to their entirely autoregressive decoding scheme, wherein the production of each new token is conditioned on all previously generated tokens. In particular, we hypothesize that top-down autoregressive decoding is disadvantageous when generating logical forms that are composed of independent subexpressions, i.e., when there are multiple subexpressions whose meanings are \textit{not} conditional on one another. 
%Here we propose an alternative method for decoding that is designed to address this notion of independence. %The decoder in our model builds up a \textit{set} of possible logical forms, rather than just a single logical form (as with top-down parsers). At each decoding step, logical forms from the set are selected to be joined together or extended with a new symbol (e.g., two entities joined together with a predicate), which allows our method to condition on only the logical expressions involved in that particular generation step. This decoding strategy would ordinarily  \cite{robinson1965machine}
%Specifically, we introduce a new neural decoding architecture that generates logical forms in a bottom-up, semi-autoregressive fashion.

In this paper, we posit that the failure of traditional neural semantic parsers to compositionally generalize is in part due to how they build logical forms. Most commonly, neural semantic parsers treat parsing as an encoder-decoder problem, where the decoder generates logical forms from the top down in an autoregressive fashion \cite{dong-lapata-2016-language,xiao-etal-2016-sequence,AlvarezMelis2017TreestructuredDW,krishnamurthy-etal-2017-neural,dong-lapata-2018-coarse}. That is, these systems output a linearization of the target logical form's abstract syntax tree, beginning from the root of the tree, where the generation of each token is conditioned on both the input text as well as the entire sequence of previously generated tokens. We propose that an entirely autoregressive decoding scheme, wherein the production of each new token is conditioned on all previously generated tokens, results in models that assume invalid dependencies to exist between tokens and thus overfit to their training data.% This overfitting is most problematic in domains where logical forms contain novel combinations of tokens and subexpressions unseen during training. 

%\achille{Is the core problem the presence of unseen sub-expressions or the fact that the traditional approach tends to force invalid dependencies on completely unrelated/independent sub-expressions? My understanding is that the core problem addressed by the bottom-up appraoch is the latter (forced dependencies). Or maybe it is both. Anyway, we need to clarify this as it is one of the core novel aspects of the new approach.}

%\maxwell{The core problem is the invalid dependencies part, I'll clarify this. The unseen combinations of subexpressions then becomes an issue when there are these unnecessary dependencies, but the core issue is the invalid dependencies.}


Here we introduce an alternative approach that eschews the top-down generation paradigm, and instead builds upwards by combining entities and subexpressions together to form larger subexpressions (Figure \ref{fig:td_bu_diff} demonstrates this distinction). Importantly, the expansion of subexpressions into larger forms is done with minimal conditioning, where only the representations of those expressions involved in the expansion are conditioned on one another for prediction. Ordinarily, such a generation strategy would be quite costly, resulting in a combinatorial explosion in the number of subexpressions created at each step; however, our approach resolves efficiency concerns by implementing a lazy evaluation scheme that allows it to selectively expand the logical form without incurring much in the way of computational overhead.

%Rather than proactively generating all possible subexpressions at each decoding step, it selectively focuses on a single subexpression at a time, generating new additions to . It  expanding from . encoding all possible subexpressions using expensive neural operations, our approach selectively builds logical forms. This lazy scheme allows our approach , separating it from other bottom-up semantic parsing approaches \cite{rubin2021smbop,odena2020bustle,Herzig2021SpanbasedSP} that  beginning from the entities. At each step in decoding, logical forms (or sub-expressions -- see Figure 1) from this set are selected to be extended with a new symbol. 

\textbf{Contributions:} In this work, we introduce a novel, bottom-up semantic parsing decoder. We show that one can simply substitute our decoder into an encoder-decoder semantic parser and achieve significant performance gains, specifically with respect to compositional generalization. We evaluate our approach on CFQ \cite{keysers2019measuring}, three Text-to-SQL \cite{finegan2018improving} datasets, and Geoquery \cite{zelle1996learning}, where we find that our approach outperforms general-purpose semantic parsers while also being competitive with comparable neural parsers that have been designed for each task.





==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old/introduction.tex <==
\section{Introduction}
\label{introduction}
% In this work, we consider the task of semantic parsing, i.e., the task of parsing a natural language utterance into a structured logical form \cite{zelle1996learning}. The earliest learning-based approaches to semantic parsing would induce probabilistic grammars that defined how words and phrases could be combined into formal meaning representations \cite{zettlemoyer2005learning,Kate2005LearningTT,kwiatkowski2011lexical}. While effective in closed domains with limited vocabularies, such approaches were often challenging to train and difficult to scale to settings involving greater breadth, e.g., WebQuestions \cite{berant2013semantic}. With the advent of deep learning and its application to natural language processing \cite{mikolov2013distributed,sutskever2014sequence}, the semantic parsing community shifted towards neural-based methods for their ability to flexibly handle language and the ease with which they could be trained.

Neural approaches to semantic parsing almost universally follow a two-stage encoder-decoder framework. In the first stage, natural language input (e.g., a question expressed in text) is encoded by a neural sequence model into a real-valued vector representation, and in the second, the encoded representation is used by a neural decoder to generate a logical form. Most commonly, the strategy followed by neural decoders is to generate logical forms from the top down in an autoregressive fashion \cite{dong-lapata-2016-language,xiao-etal-2016-sequence,AlvarezMelis2017TreestructuredDW,krishnamurthy-etal-2017-neural,dong-lapata-2018-coarse}. That is, they output a linearization of the target logical form's abstract syntax tree, beginning from the root of the tree, where the generation of each token is conditioned on both the input text as well as the entire sequence of previously generated tokens. 

While autoregressive, top-down neural semantic parsers currently hold the state-of-the-art on many challenging datasets, they have been shown to fail in systematic ways. Most notably, such systems have yet to definitively demonstrate an ability to compositionally generalize \cite{lake2018generalization,higgins2018scan}. This deficiency has been taken up as challenge by the machine learning community, leading to a slew of methods \cite{liu2021learning,herzig2021unlocking,gai2021grounded} and datasets  \cite{keysers2019measuring,kim2020cogs,johnson2017clevr} addressed specifically towards the problem of compositional generalization. However, while there has been progress in determining factors going into compositional generalization \cite{furrer2020compositional,oren2020improving}, there yet remains gaps in our understanding as to why these neural models fail.


\begin{figure}[t]
\vskip 0.2in
\begin{subfigure}{.45\textwidth}
\centering
\begin{tcolorbox}[width=\columnwidth,colback=white!95!black]
{\bf \texttt{SELECT count ( * ) WHERE \{ \\ \hspace*{1pt} ?x0 producer.film M0 .\\ \hspace*{1pt} ?x0 writer.film M0 .\\ \hspace*{1pt} M1 film.directed\_by ?x0 .\\ \hspace*{1pt} M1 film.edited\_by ?x0 \\ \} }}
\end{tcolorbox}
\end{subfigure}\hfill
\begin{subfigure}{.45\textwidth}
\centering
\begin{tcolorbox}[width=\columnwidth,colback=white!95!black]
{\bf \texttt{SELECT count ( * ) WHERE \{ \\ \hspace*{1pt} M0 film.directed\_by M1 .\\ \hspace*{1pt} M0 film.edited\_by M1 \\ \}
 }}
\end{tcolorbox}
\end{subfigure}
% \begin{subfigure}{.47\textwidth}
% \centering
% \includegraphics[width=\columnwidth]{figures/cfq_ex.png}
% \end{subfigure}
\caption{SPARQL queries for the CFQ questions "Was M1 edited by and directed by M0's writer and producer?" (left) and "Was M0 edited by and directed by M1" (right).}
\label{fig:cfq_repr}
\vskip -0.2in
\end{figure}

In this work, we posit that the failure of traditional neural semantic parsers to compositionally generalize is in part due to their entirely autoregressive decoding scheme (wherein the production of each token is conditioned on all previously generated tokens). In particular, we hypothesize that top-down autoregressive decoding is disadvantageous when generating logical forms that are composed of independent subexpressions, i.e., multiple subexpressions whose meanings are \textit{not} determined by one another. In such cases, neural models have an additional learning burden in that it must learn representations for subexpressions that reflect such an independence without any explicit signal or regularization forcing them to do so.

Here we propose an alternative that sidesteps this independence problem altogether. In our approach, the decoder builds up a \textit{set} of possible logical forms, rather than just a single logical form (as with top-down parsers). At each decoding step, logical forms from the set are selected to be joined together or extended with a new symbol (e.g., two entities joined together with a predicate), which allows our method to condition on only the logical expressions involved in that particular generation step. This decoding strategy would ordinarily  \cite{robinson1965machine}

We put our hypothesis to the test introducing and evaluating a new neural decoding architecture that generates logical forms in a bottom-up, semi-autoregressive fashion. The method we describe here is intended to be a task-agnostic replacement for top-down decoders. We show that one can simply substitute our novel decoding scheme as the decoder in for a standard autoregressive decoder to achieve significant performance gains on the challenging CFQ dataset \cite{keysers2019measuring}. With our approach, the basic LSTM goes from the worst demonstrated performance to surpassing even a fine-tuned large language model and achieving competitiveness with task-specific approaches. To demonstrate generality, we further apply our approach to the standard benchmark dataset Geoquery, where it is shown to achieve state-of-the-art performance as compared to all prior neural methods.




